Robots Pre-train Robots: Manipulation-Centric Robotic Representation from Large-Scale Robot Datasets

The pre-training of visual representations has enhanced the efficiency of robot learning. Due to the lack of large-scale in-domain robotic datasets, prior works utilize in-the-wild human videos to pre-train robotic visual representation. Despite their promising results, representations from human videos are inevitably subject to distribution shifts and lack the dynamics information crucial for task completion. We first evaluate various pre-trained representations in terms of their correlation to the downstream robotic manipulation tasks (i.e., manipulation centricity). Interestingly, we find that the "manipulation centricity" is a strong indicator of success rates when applied to downstream tasks. Drawing from these findings, we propose Manipulation Centric Representation (MCR), a foundation representation learning framework capturing both visual features and the dynamics information such as actions and proprioceptions of manipulation tasks to improve manipulation centricity. Specifically, we pre-train a visual encoder on the DROID robotic dataset and leverage motion-relevant data such as robot proprioceptive states and actions. We introduce a novel contrastive loss that aligns visual observations with the robot's proprioceptive state-action dynamics, combined with a behavior cloning (BC)-like actor loss to predict actions during pre-training, along with a time contrastive loss. Empirical results across 4 simulation domains with 20 tasks verify that MCR outperforms the strongest baseline method by 14.8%. Moreover, MCR boosts the performance of data-efficient learning with a UR5e arm on 3 real-world tasks by 76.9%. Project website: https://robots-pretrain-robots.github.io/.

==> arxiv/table/gradcam+performance.tex <==
% \begin{table*}
% \centering
% \begin{tabular}{@{}c@{\hspace{3pt}}l@{\hskip .3in}lllll@{}}\\
% \multirow{2}{*}{\textbf{Agent}} & \multirow{2}{*}{\textbf{Train Data}} & \multicolumn{3}{c}{\textbf{Test Task}} & \multirow{2}{*}{\includegraphics[width=0.05\textwidth]{figure/150x150.png}}\\
% & & \slide & \lift & \pnp  \\
% \toprule
% \multirow{4}{*}{\BC}
% & in-domain      & \underline{0.681 ± 0.147}                                  & \underline{0.823 ± 0.177}          & {\color[HTML]{FF6D01} \underline{0.818 ± 0.185}}  & \multirow{4}{*}{\includegraphics[width=0.12\textwidth]{figure/150x150.png}}\\ 
% & slide          & \underline{0.681 ± 0.147}                                  & 0.582 ± 0.058                                   & 0.612 ± 0.123                                 \\
% & slide+lift     & 0.595 ± 0.127                                 & 0.580 ± 0.053                                    & 0.605 ± 0.120                                 \\
% & slide+lift+PnP & 0.610 ± 0.137                                 & 0.609 ± 0.079                                   & 0.640 ± 0.144                                 \\
% \midrule
% \multirow{4}{*}{\MOREL}
% & in-domain      & \underline{0.629 ± 0.160}                                 & 0.678 ± 0.186                                 & 0.750 ± 0.197         & \multirow{4}{*}{\includegraphics[width=0.12\textwidth]{figure/150x150.png}}                       \\
% & slide          & \underline{0.629 ± 0.160}                                 & 0.606 ± 0.063                                 & 0.744 ± 0.174                                 \\
% & slide+lift     & 0.616 ± 0.146                                 & {\color[HTML]{46BDC6}0.726 ± 0.184}                                 & 0.636 ± 0.173                                 \\
% & slide+lift+PnP & {\color[HTML]{46BDC6} 0.715 ± 0.134}          & {\color[HTML]{46BDC6} \textbf{\underline{0.896 ± 0.133}}}          & {\color[HTML]{46BDC6} 0.753 ± 0.181}                                 \\

% \midrule
% \multirow{4}{*}{\AWAC}

% & in-domain      & \underline{0.732 ± 0.113}                                 & 0.863 ± 0.149 *                                 & 0.735 ± 0.175 *        & \multirow{4}{*}{\includegraphics[width=0.12\textwidth]{figure/150x150.png}}                        \\
% & slide          & \underline{0.732 ± 0.113}                                  & 0.638 ± 0.055                                 & {\color[HTML]{46BDC6}0.770 ± 0.111}*                                 \\
% & slide+lift     & 0.734 ± 0.110  *         & {\color[HTML]{46BDC6} 0.899 ± 0.149} & {\color[HTML]{46BDC6} \underline{0.813 ± 0.121}}          \\
% & slide+lift+PnP & 0.644 ± 0.144 *          & 0.728 ± 0.200 *   & {\color[HTML]{46BDC6}\underline{0.758 ± 0.188}} *                                 \\
% \midrule
% \multirow{4}{*}{\IQL}
% & in-domain      & {\color[HTML]{FF6D01} \textbf{\underline{0.767 ± 0.065}}} & {\color[HTML]{FF6D01} \underline{0.880 ± 0.149}}                                 & 0.601 ± 0.228           & \multirow{4}{*}{\includegraphics[width=0.12\textwidth]{figure/150x150.png}}                      \\
% & slide          & 0.767 ± 0.065                                 & 0.258 ± 0.033                                 & {\color[HTML]{46BDC6}0.810 ± 0.107}                                 \\
% & slide+lift     & 0.704 ± 0.141                                 & 0.863 ± 0.166                                 & {\color[HTML]{46BDC6} \textbf{\underline{0.842 ± 0.114}}}          \\
% & slide+lift+PnP & 0.643 ± 0.143                                 & 0.684 ± 0.158                                 & {\color[HTML]{46BDC6}\underline{0.833 ± 0.183}}  \\
% \bottomrule
% \end{tabular}
% \vspace{2mm}
% \caption{Performance of agents trained with different combinations of offline data. \textcolor{orange}{The best in-domain agent}, \textcolor{cyan}{transfer learning agents that improves over their in-domain counterparts} are colored. The \textbf{best agent for each task} is bold. Agents that could not converge during training time are marked with (*). Some agents triggered violent crashes at test time and we report such performance as \textless 0. \underline{Underline scores} are swept over 3 seeds.}
% \label{tab:gen_combo}
% % \vspace{-1em}

% \end{table*}

     % \multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Office Environment}} & \multicolumn{2}{c|}{\textbf{Kitchen Environment}} & \multicolumn{2}{c}{\textbf{CALVIN Environment}}\\ [0ex] \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} & Succ. Rate  & Comp. Subtasks  &  Succ. Rate  & Comp. Subtasks   & Succ. Rate  & Comp. Subtasks\\

\begin{table}[t]
\begin{center}
% \vspace{-0.1in}
\caption{\textbf{Grad-CAM visualization.} 
We present Grad-CAM visualizations alongside their corresponding task success rates for the Square task from Robomimic and the Pick Place Wall task from MetaWorld. Representations that capture the robot's end-effectors and task-relevant objects are linked to improved downstream performance. Comprehensive visualizations can be found in \cref{appsec:metric}.}
\label{tab:gradcam+IL}

% \vspace{-0.1in}
\resizebox{1\textwidth}{!}{%
\setlength{\tabcolsep}{2pt}
\begin{tabular}{>{\centering\arraybackslash}m{0.01\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>
{\centering\arraybackslash}m{0.14\linewidth}>
{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}}
\toprule
& \multirow{2}[-4]{*}{Task}  & \textcolor{gpurple}{$\blacksquare$}MVP & \textcolor{gblue}{$\blacksquare$}VC-1  & \textcolor{ggreen}{$\blacksquare$}HRP & \textcolor{gyellow}{$\blacksquare$}R3M & \textcolor{gblack}{$\blacksquare$}R3M-DROID & \textcolor{gred}{$\blacksquare$}\ours & IL Score (\%)  \\
[-0.2mm]\midrule \noalign{\vskip -0.1ex}
\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Square}}}}&
% \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
\includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_ori_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_mvp_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_vc1_vitb_10.png}
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_hrp_vitb_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_r3m_50_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_r3m_50_droid_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_ours_10.png}
& \includegraphics[width=1\linewidth]{figure/robomimic_result.pdf} 
\\ %[-1mm]

% % \noalign{\vskip -0.8ex}\midrule\noalign{\vskip -0.2ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering {\small Faucet}}}}&
% % \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
% \includegraphics[width=1\linewidth]
% {figure/gradcam/faucet_10.pdf} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_mvp_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_vc1_vitb_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_hrp_vitb_10.png}
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_r3m_50_10.png} 
% &
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_ours_10.png}
% & \includegraphics[width=1\linewidth]{figure/dexart_result.pdf} 
% \\[-1mm]

% \noalign{\vskip -0.8ex}\midrule\noalign{\vskip -0.2ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{12mm}{ {\footnotesize Pick Place}}}}
\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{7mm}{\centering{\small P\&P~Wall}}}}&
% \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
\includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_ori_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_mvp_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_vc1_vitb_70.png}
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_hrp_vitb_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_r3m_50_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_r3m_50_droid_70.png}
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_ours_70.png}
& \includegraphics[width=1\linewidth]{figure/metaworld_result.pdf}
\\
\noalign{\vskip -0.5ex}
\bottomrule
    \end{tabular}}
\end{center}
% \vspace{-1em}
\vspace{-0.2in}
\end{table}


% \begin{table}
% \begin{center}

% \resizebox{0.95\textwidth}{!}{%
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{2}{c}{\multirow{2}[2]{*}{\textbf{Task}}} & \multicolumn{5}{c|}{\textbf{Grad-CAM of Representations}} & \textbf{Downstream}\\[0.4mm]
% % \cmidrule(lr){2-6} 
% &  & \textcolor{gpurple}{$\blacksquare$}MVP & \textcolor{gblue}{$\blacksquare$}VC-1  & \textcolor{gyellow}{$\blacksquare$}R3M & \textcolor{brown}{$\blacksquare$}Hrp & \textcolor{gred}{$\blacksquare$}Ours & \textbf{Success} (\%)  \\
% \midrule \noalign{\vskip -0.5ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Square}}}}&
% % \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
% \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_15.pdf} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_mvp.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_vc1_vitb.png}
% & \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_r3m_50.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_hrp_vitb.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_ours.png}
% & \includegraphics[width=1\linewidth]{figure/robomimic_result.pdf} \\
% \noalign{\vskip -0.8ex}\midrule\noalign{\vskip -0.2ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering {\small Faucet}}}}&
% % \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
% \includegraphics[width=1\linewidth]
% {figure/gradcam/faucet_10.pdf} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_mvp_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_vc1_vitb_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_r3m_50_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_hrp_vitb_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_ours_10.png}
% & \includegraphics[width=1\linewidth]{figure/dexart_result.pdf} \\
% \noalign{\vskip -0.8ex}\midrule\noalign{\vskip -0.2ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{9.5mm}{ {\small Disassemble}}}}&
% % \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
% \includegraphics[width=1\linewidth]{figure/gradcam/disassemble_60.pdf} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/disassemble_mvp_60.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/disassemble_vc1_vitb_60.png}
% & \includegraphics[width=1\linewidth]{figure/gradcam/disassemble_r3m_50_60.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/disassemble_hrp_vitb_60.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/disassemble_ours_60.png}
% & \includegraphics[width=1\linewidth]{figure/robomimic_result.pdf} \\
% \noalign{\vskip -0.5ex}
% \bottomrule
% \end{tabular}}
% \end{center}
% \caption{This table provides Grad-CAM visualization and IL performance, aiming to provide rough insight on manipulation centricity. Choose 3 representative tasks. Put Grad-CAM in column 2-6. Put the IL score (bar plot) in column 7. Note the color of the legend in the IL score figure should be consistent with the ones in this table. Change the color here to ours @gq\&yf. \guangqi{maybe choose tasks that fit the correlation between cam and success}} 
% \label{tab:gradcam+IL}
% % \vspace{-1em}
% \end{table}

==> table/each_task_result.tex <==
\begin{table*}[htbp]
\centering
\caption{\textbf{Main results on 20 simulation tasks.} Results for each task are provided in this table. A summary across domains is shown in Figure~\ref{fig:real_task_visualization}. \guangqi{@yf update if requested}}
\label{table: simulation results}
\begin{flushleft}
\resizebox{1.0\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cccc|ccc|ccc}
\toprule
& \multicolumn{4}{c|}{\textbf{DexArt}}& \multicolumn{3}{c|}{\textbf{Robomimic}} & \multicolumn{3}{c}{\textbf{RobocCasa}}
\\

 Alg $\backslash$ Task & Bucket & Faucet & Laptop  & Toilet & Can &Lift & Square & CloseDrawer& CoffeeButtonPress & OpenSingleDoor  \\

\midrule
\ourrow \ours~(ours) & 36.7\ci{2.9} & 38.3\ci{2.9} & 93.3\ci{2.9} & 73.3\ci{2.9} & 68.0\ci{4.0} & 96.0\ci{2.3} & 30.0\ci{1.2} & 99.3\ci{1.2} & 72.0\ci{3.5} & 56.0\ci{3.5} \\
LfS & 33.3\ci{5.8} & 36.7\ci{5.8} & 83.3\ci{10.4} & 71.7\ci{2.9} & 6.0\ci{0.0} & 64.0\ci{4.2} & 4.0\ci{0.0} & 85.3\ci{1.2} & 52.0\ci{4.0} & 46.7\ci{1.2} \\
MVP & 31.7\ci{2.9} & 33.3\ci{2.9} & 81.7\ci{5.8} & 80.0\ci{0.0} & 28.0\ci{2.0} & 74.0\ci{6.4} & 14.0\ci{2.3} & 98.0\ci{2.0} & 52.7\ci{18.9} & 33.3\ci{14.5} \\
VC1 & 30.0\ci{0.0} & 35.0\ci{0.0} & 85.0\ci{0.0} & 71.7\ci{2.9} & 44.0\ci{7.0} & 74.0\ci{9.2} & 20.0\ci{3.5} & 98.7\ci{2.0} & 29.3\ci{5.8} & 33.3\ci{7.0} \\
R3M & 31.7\ci{2.9} & 36.7\ci{2.9} & 81.7\ci{5.8} & 71.7\ci{2.9} & 50.0\ci{4.2} & 86.0\ci{6.0} & 24.0\ci{1.2} & 88.7\ci{3.1} & 47.3\ci{6.1} & 48.7\ci{7.6} \\
HRP & 31.7\ci{2.9} & 36.7\ci{2.9} & 90.0\ci{5.0} & 63.3\ci{14.4} & 42.0\ci{3.5} & 86.0\ci{3.5} & 26.0\ci{2.3} & 91.3\ci{4.6} & 35.3\ci{11.6} & 38.0\ci{6.0} \\
R3M-Droid & 35.0\ci{5.0} & 33.3\ci{2.9} & 80.0\ci{0.0} & 66.7\ci{7.6} & 54.0\ci{2.3} & 96.0\ci{0.0} & 22.0\ci{3.1} & 88.7\ci{2.3} & 51.3\ci{2.3} & 45.3\ci{7.6} \\




\end{tabular}}

\resizebox{1.0\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cc|cc|c|ccccc}
\toprule
& \multicolumn{2}{c|}{\textbf{MetaWorld}}&  \multicolumn{2}{c|}{\textbf{MetaWorld (Medium)} }& \multicolumn{1}{c|}{\textbf{MetaWorld (Hard)} }&\multicolumn{5}{c}{\textbf{MetaWorld (Very Hard)}}
\\

 Alg $\backslash$ Task &  Button Press & Drawer Open &Bin Picking & Hammer &Assembly & Shelf Place & Disassemble & Stick Pull & Stick Push & Pick Place Wall\\

\midrule

\ourrow \ours~(ours) & 100.0\ci{0.0} & 100.0\ci{0.0} & 96.7\ci{2.9} & 100.0\ci{0.0} & 100.0\ci{0.0} & 41.7\ci{5.8} & 93.3\ci{2.9} & 86.7\ci{2.9} & 100.0\ci{0.0} & 91.7\ci{2.9} \\

LfS & 96.7\ci{2.9} & 95.0\ci{5.0} & 81.7\ci{2.9} & 95.0\ci{5.0} & 95.0\ci{5.0} & 35.0\ci{5.0} & 86.7\ci{2.9} & 83.3\ci{5.8} & 96.7\ci{2.9} & 85.0\ci{5.0} \\

MVP & 96.7\ci{2.9} & 98.3\ci{2.9} & 81.7\ci{2.9} & 91.7\ci{2.9} & 86.7\ci{2.9} & 20.0\ci{5.0} & 65.0\ci{8.7} & 75.0\ci{8.7} & 96.7\ci{2.9} & 76.7\ci{11.6} \\

VC-1 & 98.3\ci{2.9} & 98.3\ci{2.9} & 78.3\ci{2.9} & 86.7\ci{2.9} & 95.0\ci{5.0} & 21.7\ci{2.9} & 66.7\ci{2.9} & 86.7\ci{2.9} & 98.3\ci{2.9} & 71.7\ci{2.9} \\

R3M & 91.7\ci{2.9} & 71.7\ci{16.1} & 21.7\ci{2.9} & 63.3\ci{5.8} & 36.7\ci{2.9} & 35.0\ci{8.7} & 76.7\ci{2.9} & 43.3\ci{7.6} & 71.7\ci{2.9} & 58.3\ci{5.8} \\

HRP & 98.3\ci{2.9} & 98.3\ci{2.9} & 90.0\ci{0.0} & 65.0\ci{0.0} & 96.7\ci{2.9} & 23.3\ci{2.9} & 61.7\ci{2.9} & 85.0\ci{0.0} & 96.7\ci{2.9} & 81.7\ci{2.9} \\

R3M-Droid & 98.3\ci{2.9} & 96.7\ci{5.8} & 90.0\ci{0.0} & 80.0\ci{0.0} & 83.3\ci{5.8} & 38.3\ci{2.9} & 66.7\ci{2.9} & 61.7\ci{20.2} & 98.3\ci{2.9} & 83.3\ci{5.8} \\


\bottomrule

\end{tabular}}

\end{flushleft}
\end{table*}

==> table/gradcam_all.tex <==
\setlength{\tabcolsep}{0.6 mm}
 \begin{longtable}{
 >{\centering\arraybackslash}m{0.01\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}
 }

\caption{\textbf{Grad-CAM of all tasks} \guangqi{@yf, add one column of manipulation centricity segmentation mask, adjust so that the table does not exceed right margin (now it exceeds)}} \label{tab:gradcam+IL_all} \\ % 将标题放在 longtable 外
\toprule

& \multirow{2}[-4]{*}{Task}  & \textcolor{gpurple}{$\blacksquare$}MVP & \textcolor{gblue}{$\blacksquare$}VC-1  & \textcolor{ggreen}{$\blacksquare$}HRP & \textcolor{gyellow}{$\blacksquare$}R3M & \textcolor{gblack}{$\blacksquare$}R3M-DROID & \textcolor{gred}{$\blacksquare$}\ours \\
[-0.2mm]\midrule
\endfirsthead

\caption[]{\textbf{Grad-CAM of all tasks}} \\ % 每页的表头

\toprule
& \multirow{2}[-4]{*}{Task}  & \textcolor{gpurple}{$\blacksquare$}MVP & \textcolor{gblue}{$\blacksquare$}VC-1  & \textcolor{ggreen}{$\blacksquare$}HRP & \textcolor{gyellow}{$\blacksquare$}R3M & \textcolor{gblack}{$\blacksquare$}R3M-DROID & \textcolor{gred}{$\blacksquare$}\ours \\
[-0.2mm]\midrule
\endhead

\midrule \multicolumn{8}{r}{Continue} \\ % 每页的表尾
\endfoot

\bottomrule % 最后一页的表尾
\endlastfoot


\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Can}}}}&
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_16.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_gradcam_mvp_cam_output_16.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_gradcam_vc1_vitb_cam_output_16.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_gradcam_hrp_vitb_cam_output_16.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_gradcam_r3m_50_cam_output_16.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_gradcam_r3m_50_droid_cam_output_16.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_can_gradcam_ours_cam_output_16.jpg} \\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Lift}}}}&
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_3.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_gradcam_mvp_cam_output_3.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_gradcam_vc1_vitb_cam_output_3.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_gradcam_hrp_vitb_cam_output_3.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_gradcam_r3m_50_cam_output_3.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_gradcam_r3m_50_droid_cam_output_3.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robomimic_lift_gradcam_ours_cam_output_3.jpg} \\


\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}
{\centering{\small Square}}}}&
\includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_ori_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_mvp_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_vc1_vitb_10.png}
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_hrp_vitb_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_r3m_50_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_r3m_50_droid_10.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/robomimic_square_ours_10.png}\\


\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{8mm}{\centering{\small CloseDrawer}}}}&
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_20.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_gradcam_mvp_cam_output_20.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_gradcam_vc1_vitb_cam_output_20.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_gradcam_hrp_vitb_cam_output_20.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_gradcam_r3m_50_cam_output_20.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_gradcam_r3m_50_droid_cam_output_20.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CloseDrawer_gradcam_ours_cam_output_20.jpg} \\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{12mm}{\centering{\small CoffeePressButton}}}}&
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_40.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_gradcam_mvp_cam_output_40.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_gradcam_vc1_vitb_cam_output_40.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_gradcam_hrp_vitb_cam_output_40.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_gradcam_r3m_50_cam_output_40.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_gradcam_r3m_50_droid_cam_output_40.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_CoffeePressButton_gradcam_ours_cam_output_40.jpg} \\


\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{13mm}{\centering{\small OpenSingleDoor}}}}&
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/robocasa_OpenSingleDoor_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Assembly}}}}&
% \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Assembly}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/assembly_gradcam_ours_cam_output_10.jpg}
\\ %[-1mm]

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{8mm}{\centering{\small BinPicking}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bin-picking_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{9mm}{\centering{\small ButtonPress}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_70.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_gradcam_mvp_cam_output_70.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_gradcam_vc1_vitb_cam_output_70.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_gradcam_hrp_vitb_cam_output_70.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_gradcam_r3m_50_cam_output_70.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_gradcam_r3m_50_droid_cam_output_70.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/button-press_gradcam_ours_cam_output_70.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{9mm}{\centering{\small Disassemble}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/disassemble_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{9mm}{\centering{\small DrawerOpen}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/drawer-open_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Hammer}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_60.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_gradcam_mvp_cam_output_60.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_gradcam_vc1_vitb_cam_output_60.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_gradcam_hrp_vitb_cam_output_60.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_gradcam_r3m_50_cam_output_60.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_gradcam_r3m_50_droid_cam_output_60.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/hammer_gradcam_ours_cam_output_60.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{10mm}{\centering{\small PickPlaceWall}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_ori_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_mvp_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_vc1_vitb_70.png}
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_hrp_vitb_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_r3m_50_70.png} 
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_r3m_50_droid_70.png}
& \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_ours_70.png}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{9mm}{\centering{\small ShelfPlace}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_100.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_gradcam_mvp_cam_output_100.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_gradcam_vc1_vitb_cam_output_100.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_gradcam_hrp_vitb_cam_output_100.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_gradcam_r3m_50_cam_output_100.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_gradcam_r3m_50_droid_cam_output_100.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/shelf-place_gradcam_ours_cam_output_100.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{8mm}{\centering{\small StickPull}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-pull_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{8mm}{\centering{\small StickPush}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/stick-push_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Bucket}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/bucket_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Faucet}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/faucet_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Laptop}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/laptop_gradcam_ours_cam_output_10.jpg}
\\

\multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering{\small Toilet}}}} &
\includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_10.jpg} 
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_gradcam_mvp_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_gradcam_vc1_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_gradcam_hrp_vitb_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_gradcam_r3m_50_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_gradcam_r3m_50_droid_cam_output_10.jpg}
& \includegraphics[width=1\linewidth]{figure/gradcam_image_cut/toilet_gradcam_ours_cam_output_10.jpg}
\\

% % \noalign{\vskip -0.8ex}\midrule\noalign{\vskip -0.2ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{6mm}{\centering {\small Faucet}}}}&
% % \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
% \includegraphics[width=1\linewidth]
% {figure/gradcam/faucet_10.pdf} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_mvp_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_vc1_vitb_10.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_hrp_vitb_10.png}
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_r3m_50_10.png} 
% &
% & \includegraphics[width=1\linewidth]{figure/gradcam/faucet_ours_10.png}
% & \includegraphics[width=1\linewidth]{figure/dexart_result.pdf} 
% \\[-1mm]

% \noalign{\vskip -0.8ex}\midrule\noalign{\vskip -0.2ex}
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\parbox[c]{9.5mm}{ {\footnotesize Pick Place}}}}&
% % \parbox[c]{20mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Disassemble}}} &
% \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_ori_70.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_mvp_70.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_vc1_vitb_70.png}
% & \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_hrp_vitb_70.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_r3m_50_70.png} 
% & \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_r3m_50_droid_70.png}
% & \includegraphics[width=1\linewidth]{figure/gradcam/pick-place-wall_ours_70.png}
% \\

\noalign{\vskip -0.5ex}
\bottomrule

\end{longtable}

==> table/main_realworld.tex <==
% \begin{figure}[!ht]
% \vspace{1em}
%     \centering
%     \begin{minipage}[t]{0.6\linewidth}
%         \vspace{0pt}
%         \centering
%         \setlength{\tabcolsep}{1mm}  
%         % \renewcommand{\arraystretch}{1.5}
%         % \normalsize  % 使用 \normalsize 作为中间选择
%         \begin{tabular}{@{}lccccc@{}}  
%         \toprule
%           Task & LfS & MVP  & VC-1 &  R3M & \textbf{\ours} \\
%         \midrule
%         Lift & \scalebox{1.5}{\sfrac{5}{10}} & \scalebox{1.5}{\sfrac{6}{10}} & \scalebox{1.5}{\sfrac{5}{10}} & \scalebox{1.5}{\sfrac{6}{10}} & \textbf{\scalebox{1.5}{\sfrac{9}{10}}}\\[3pt]
%         Sweep & \scalebox{1.5}{\sfrac{3}{10}} & \scalebox{1.5}{\sfrac{1}{10}} & \scalebox{1.5}{\sfrac{2}{10}} & \scalebox{1.5}{\sfrac{1}{10}} & \textbf{\scalebox{1.5}{\sfrac{7}{10}}} \\[3pt]
%         Rearrange & \scalebox{1.5}{\sfrac{2}{10}} & \scalebox{1.5}{\sfrac{3}{10}} & \scalebox{1.5}{\sfrac{6}{10}} & \scalebox{1.5}{\sfrac{4}{10}} & \textbf{\scalebox{1.5}{\sfrac{7}{10}}} \\[3pt]
%         \midrule
%         All & \scalebox{1.5}{\sfrac{10}{30}} & \scalebox{1.5}{\sfrac{10}{30}} & \scalebox{1.5}{\sfrac{13}{30}} & \scalebox{1.5}{\sfrac{11}{30}} &  \textbf{\scalebox{1.5}{\sfrac{23}{30}}}\\
%         \bottomrule
%         \end{tabular}
%     \end{minipage}
%     \begin{minipage}[t]{0.38\linewidth}
%         \vspace{0pt}
%         \centering
%         \includegraphics[width=\linewidth]{figure/real_gradcam.pdf}
%     \end{minipage}%
%     \hfill
%     \captionlistentry[table]{A table beside a figure}
%     \captionsetup{labelformat=andtable}
%     \caption{\textbf{Real robot results.} Each task is fairly assessed over 10 trials. Our method (\ours) performs best in all tasks.}
% \end{figure}

\begin{figure}[!ht]
\vspace{1em}
    \centering
    \vspace{-0.23in}
    \begin{minipage}[t]{0.62\linewidth}
        \vspace{0pt}
        \centering
    \resizebox{1\linewidth}{!}{
    \setlength{\tabcolsep}{11pt}
        % \renewcommand{\arraystretch}{1.5}
        % \normalsize  % 使用 \normalsize 作为中间选择
        \begin{tabular}{@{}lccccc@{}}  
        \toprule
          Task & LfS & MVP  & VC-1 &  R3M & \ours \\
        \midrule
        Lift & \scalebox{1.5}{\sfrac{5}{10}} & \scalebox{1.5}{\sfrac{6}{10}} & \scalebox{1.5}{\sfrac{5}{10}} & \scalebox{1.5}{\sfrac{6}{10}} & \textbf{\scalebox{1.5}{\sfrac{9}{10}}}\\[0pt]
        Sweep & \scalebox{1.5}{\sfrac{3}{10}} & \scalebox{1.5}{\sfrac{1}{10}} & \scalebox{1.5}{\sfrac{2}{10}} & \scalebox{1.5}{\sfrac{1}{10}} & \textbf{\scalebox{1.5}{\sfrac{7}{10}}} \\[0pt]
        Rearrange & \scalebox{1.5}{\sfrac{2}{10}} & \scalebox{1.5}{\sfrac{3}{10}} & \scalebox{1.5}{\sfrac{6}{10}} & \scalebox{1.5}{\sfrac{4}{10}} & \textbf{\scalebox{1.5}{\sfrac{7}{10}}} \\[0pt]
        \midrule
        All & \scalebox{1.5}{\sfrac{10}{30}} & \scalebox{1.5}{\sfrac{10}{30}} & \scalebox{1.5}{\sfrac{13}{30}} & \scalebox{1.5}{\sfrac{11}{30}} &  \textbf{\scalebox{1.5}{\sfrac{23}{30}}}\\
        \bottomrule        
        \end{tabular}}
        \vspace{-0.1in}
         \captionof{table}{\textbf{Real robot results.} Our method \ours~performs best in all tasks. Each method is fairly assessed over 10 trials on each task.}\label{table:real_robot}
    \end{minipage}
    \captionlistentry[table]{A table beside a figure}
    \hfill
    \begin{minipage}[t]{0.37\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=0.92\linewidth]{arxiv/figure/real_gradcam.pdf}\label{fig:real_gradcam}
        \vspace{-0.1in}
        \captionof{figure}{\textbf{Grad-CAM on Rearrange.} \ours~is with best manipulation centricty.}
    \end{minipage}%
    % \caption{\textbf{Real robot results.} Each task is fairly assessed over 10 trials.\label{fig+table} (\textbf{Left}) Our method \ours performs best in all tasks. (\textbf{right}) The }
    \vspace{-0.1in}
\end{figure}
